FLSys: Toward an Open Ecosystem for Federated Learning Mobile Apps

This article presents the design, implementation, and evaluation of FLSys, a mobile-cloud federated learning (FL) system, which can be a key component for an open ecosystem of FL models and apps. FLSys is designed to work on smart phones with mobile sensing data. It balances model performance with resource consumption, tolerates communication failures, and achieves scalability. In FLSys, different DL models with different FL aggregation methods can be trained and accessed concurrently by different apps. Furthermore, FLSys provides advanced privacy preserving mechanisms and a common API for third-party app developers to access FL models. FLSys adopts a modular design and is implemented in Android and AWS cloud. We co-designed FLSys with a human activity recognition (HAR) model. HAR sensing data was collected in the wild from 100+ college students during a 4-month period. We implemented HAR-Wild, a CNN model tailored to mobile devices, with a data augmentation mechanism to mitigate the problem of non-Independent and Identically Distributed data. A sentiment analysis model is also used to demonstrate that FLSys effectively supports concurrent models. This article reports our experience and lessons learned from conducting extensive experiments using simulations, Android/Linux emulations, and Android phones that demonstrate FLSys achieves good model utility and practical system performance.

==> alter_sec7_data_collection.tex <==
\section{Data Collection}
\label{sec:data_collection}
{\fontfamily{ptm}\selectfont

\subsection{HAR Data Collection Details}

Through our Data Collector, we collect smartphone sensor data (Table \ref{SensorData}) ``in the wild'' from university students as subjects. We launched two data collection runs at two U.S. universities for three months each. During the course of three months, we ask the participants to collect data and labels by themselves (in the wild), and only intervene through reminding emails if we saw a decline in the amount of daily activities. A total of 116 participants with valid data were recorded after the two data collection runs. 

\begin{wrapfigure}{l}{0.18\textwidth}
  \begin{center} \vspace{-20pt}
    \includegraphics[width=0.2\textwidth]{image/Screenshot_anoymous.png} \vspace{-30pt}
  \end{center}
  \caption{Data Collector labeling interface.} \vspace{-10pt}
  \label{data_collector_labeling_interface}
\end{wrapfigure}

\begin{table*}[t]
\small
\centering
\caption{Types of Sensor Data Collected}
\begin{tabular}{|l|l|l|l|l|}
\hline
Sensor                             & Type                                    & Sampling rate                      & Availability                     & Description                                                                               \\ \hline
Accelerometer                      & Motion                           & 5Hz $\sim$50Hz                     & 114/116                          & Measures the linear acceleration   (including gravity)                                    \\
Gyroscope                          & Motion                           & 5Hz                                & 114/116                          & Measures the angular speed                                                                \\
Rotation                           & Motion                           & 5Hz                                & 114/116                          & Provides the rotation vector   component                                                  \\
GPS                                & Position                         & Variable                           & 110/116                          & Typical GPS data                                                                          \\
Magnetometer                       & Position                         & 5Hz                                & 113/116                          & Measures the geomagnetic field   strength                                                 \\
Pressure                           & Environment                      & 5Hz                                & 83/116                           & Measures ambient air pressure                                                             \\
Light                              & Environment                      & Variable                           & 110/116                          & Measures ambient light level   (illumination)                                             \\
Battery log                        & Phone state                      & Variable                           & 116/116                          & Measures the smartphone’s battery   level                                                 \\
Proximity                          & Phone state                      & Variable                           & 109/116                          & Measures the distance between the   screen and an object                                  \\
Power state                        & Phone state                      & Variable                           & 115/116                          & Different values indicating   different state/event of the smartphone                     \\
Call log                           & User data                               &                                    & 98/116                           & Logs the calls that the user had                                                          \\
SMS log                            & User data                               &                                    & 98/116                           & Logs the short messages (SMS) that   the user had                                         \\
\hline
\multicolumn{5}{|l|}{\begin{tabular}[c]{@{}l@{}}*The sampling rate is estimated   from observation, actual values vary\\ **The availability means that out   of the 116 participants, how many of them provided this data type 
\end{tabular}}
\\ \hline
\end{tabular}
\label{SensorData}
\end{table*}

\begin{table*}[]
\small
\centering
\caption{Total time of sensor sessions (continuous sensors)}
\begin{tabular}{|llllllll|}
\hline
Sensor        & Total\_time & 60hz\_up  & 50hz      & 40hz   & 20hz     & 5hz        & The\_rest \\ \hline
Accelerometer & 2278050.17  & 120056.98 & 241932.44 & 642.59 & 69136.15 & 1012894.06 & 833387.95 \\
Gyroscope     & 2273397.28  & 110149.8  & 15448.17  & 7.39   & 31354.51 & 1795766.05 & 320671.36 \\
Rotation      & 2290372.31  & 23073.62  & 71003.64  & 441.01 & 33341.33 & 2061158.39 & 101354.32 \\
Magnetometer  & 2287446.51  & 870.32    & 4058.21   & 0      & 23.01    & 2193983.48 & 88511.49  \\ \hline
\multicolumn{8}{|l|}{*In a number of minutes}                                                    \\
\multicolumn{8}{|l|}{**Only count data sessions at least   30 seconds long}                      \\ \hline
\end{tabular}
\label{SensorSessions}
\end{table*}

The types of data that the app can collect are listed in Table \ref{SensorData}. In Table \ref{SensorSessions}, we show the total number of minutes of data collected from the four types of sensors that collects continuous (relatively continuous compared with other sensors that collect data points at a much lower rate or at certain events) data sessions. We can see that only the Accelerometer collected a meaningful amount of data at the sampling rate higher than 5Hz. 

% Table \ref{} shows the number of data points collected from the rest of the sensors. Note that the Pressure sensor and the Light sensor collect data points at regular (but low) rates, while other sensors at certain events.

\begin{comment}
\begin{figure}[t!]
  \centering
  \includegraphics[width=0.4\linewidth]{image/Screenshot_anoymous.png}
  \caption{Data Collector labeling interface.}
  \label{data_collector_labeling_interface}
\end{figure}
\end{comment}


\begin{comment}
\begin{table}[t]
\small
\centering
\caption{Total number of data points (non-continuous sensors)}
\begin{tabular}{|l|l|}
\hline
Sensor     & Total number of data points \\ \hline
gps        & 1251970                     \\ \hline
pressure   & 971782334                   \\ \hline
light      & 380064951                   \\ \hline
batteryLog & 7721722                     \\ \hline
proximity  & 3280332                     \\ \hline
powerState & 794895                      \\ \hline
callLog    & 11362                       \\ \hline
textsLog   & 204728                      \\ \hline
\end{tabular}
\end{table}
\end{comment}

\begin{table}[t]
\small
\caption{Labels and the total number of minutes collected for each label}
\begin{tabular}{|l|l|l|}
\hline
Type           & Label                        & Total minutes \\ \hline
Activity       & sitting                      & 862544.50     \\ \hline
               & walking                      & 158087.40     \\ \hline
               & driving                      & 38013.98      \\ \hline
               & lying                        & 488596.70     \\ \hline
               & cycling                      & 2589.50       \\ \hline
               & workout\_gym                 & 3649.47       \\ \hline
               & workout\_running             & 2212.69       \\ \hline
               & workout\_others              & 16500.13      \\ \hline
               & workout\_recreational sports & 0.00          \\ \hline
Phone position & palm                         & 511092.20     \\ \hline
               & bag                          & 6446.19       \\ \hline
               & pocket                       & 99557.67      \\ \hline
               & table                        & 864904.00     \\ \hline
               & mounted                      & 49440.29      \\ \hline
               & strap                        & 2485.22       \\ \hline
User location  & vehicle\_car                 & 72121.55      \\ \hline
               & vehicle\_train/subway        & 355.24        \\ \hline
               & vehicle\_plane               & 0.00          \\ \hline
               & vehicle\_bus/shuttle         & 0.00          \\ \hline
               & vehicle\_motorcycle          & 88.84         \\ \hline
               & home                         & 1171968.00    \\ \hline
               & outside                      & 41886.80      \\ \hline
               & travel                       & 14094.12      \\ \hline
               & elevator                     & 924.09        \\ \hline
               & office                       & 17562.08      \\ \hline
\end{tabular}
\label{DataActivities}
\end{table}

Regarding labels of activities, we provide a simple interface in our Data Collector for users to quickly select the appropriate labels, as shown in Figure \ref{data_collector_labeling_interface}. We summarized the labels into three categories: (1) Physical activity; (2) Phone position; and (3) User location. Each category has several pre-defined sub-types for users to choose from. The details can be seen in Table \ref{DataActivities}. Reported activities cover a vast majority of daily activities that are of research interests. Users can choose the labeling to last either for a defined time length (e.g., 5 minutes, 10 minutes, or 20 minutes) or for an unlimited time (i.e., in this case, users need to remember to turn off the label when the activity is done). We can see that the distribution of user activities is consistent with the ``stay home order'' during the COVID-19 pandemic.

\subsection{Data Processing}

%  Although our Data Collector is designed to be battery efficient, data collection in the wild, especially for human activity recognition (HAR), is noisy and more complicated than in well-controlled environments. This introduces inconsistency across data sessions used for a labeled human activity.
% given an unfixed high frequency of sensor sampling rates

% To cope with this challenge, the data processing steps need to achieve three objectives: \textbf{(1)} Remove or fix the errors and imperfections in the raw data, including repeated data points, gaps between data points, fluctuating sampling rates, and inaccurate labels; \textbf{(2)} Align the sensor data with the labels across time, such that each unit of data points is associated with its correct label; and \textbf{(3)} Convert the format of the raw data into short sessions of data points with multiple channels (i.e., accelerometer data has 3 channels, x, y, z, in the data representation) that will serve as basic input data units of the deep learning models. 

The goal of data processing is to have the data ready to be consumed by the deep learning models. To make our Data Collector less invasive to test subjects' daily life (less impact of battery life, and less interrupting), we had to make compromises, e.g. lower sampling rates and noisy (inconsistent) labels. To cope with this challenge, we design the data processing steps with three objectives: (1) Fix or mitigate the errors and imperfections in the raw sensor data, including gaps, repetitive data points and fluctuating sampling rates; (2) Identify and remove inconsistency in the labels; and (3) Convert the raw data into short segments of data points (data matrix) with shape $[3, 100]$, that are the basic input data units for DL models, where each data segment consists of 100 3-axis data points of Accel data. The exact steps are shown as follow:

\begin{itemize}
    \item Step 1: Any duplicated data points (e.g., data points that have the same timestamp) are merged by taking the average of their sensor values.
    \item Step 2: Using 300 milliseconds as the threshold, continuous data sessions are identified and separated by breaking up the data sequences at any gap that is larger than the threshold. This threshold is relatively strict, and it is defined based on the lowest effective sampling rate (5Hz) with some flexibility so that data sessions are not broken into too many pieces.
    \item Step 3: Data sessions that have unstable or unsuitable sampling rates are filtered out. We only keep the data sessions that have a stable sampling rate of 5Hz or 20Hz or 50Hz. To achieve this, key statistics that are related to the sampling rate of each session, including the mean, the variance, and the 50\% quantile of the sampling intervals, are computed. Then, the sessions that meet all of the following criteria are kept as potential valid data sessions: (a) The mean sampling rate (computed from mean sampling interval) falls within ±25\% of the target sampling rates; (b) The 50\% quantile sampling rate (computed from 50\% quantile sampling interval) falls within ±25\% of the target sampling rates; (c) The total duration exceeds 30 seconds. Here the assumption is that if the mean sampling rate and the 50\% quantile sampling rate agrees, it indicates that the data session has a relatively stable sampling rate. We keep each data session at their original sampling rate.
    \item Step 4: The label session(s) that are associated with each data session (if any) are identified from the raw labels data. Note that the label sessions are also filtered with the following two criteria to ensure good quality: (a) The first 10 seconds and the last 10 seconds of each label session are trimmed, due to the fact that users were likely operating the phone during these time periods; (b) Any label session longer than 30 minutes is trimmed down to the first 30 minutes, in order to mitigate the potential inaccurate labels due to users’ negligence (forgot to turn off labeling).
    \item Step 5: We sample data segments at the size of 100 data points with sliding windows. Different overlapping percentages were used for different classes. The majority classes have 25\% overlapping, while the minority classes have up to 90\% overlapping. All data segments with different sampling rates are mixed together, without distinguishing between them. We sample 15\% of data for testing, with the guarantee that training and testing data never overlaps. The rest 85\% of data points are used for training. The statistics of the dataset are also shown in Table \ref{tab:dataset}.
    \item Step 6: All the sensor values are normalized with z-score using the mean and standard deviation computed from the training dataset. This step is a common practice that helps to stabilize the gradients during training.
    \item Step 7: Finally, we compute the mean-variance on each data segment with a rolling window (window size = 20), then filter out any data segment that has a variance value less than the threshold of 0.001. This step filters out the “flat” data segments that are labeling errors (since all of our classes represents some type of movement).
\end{itemize}

}

==> data.tex <==
\section{Data Collection, Processing, and Statistics}
\label{sec:data}
{\fontfamily{ptm}\selectfont
 
 
Although our Data Collector for sensor data is designed to be battery efficient, data collection in the wild, especially for human activity recognition (HAR), is noisy and more complicated than in well-controlled environments given an unfixed high frequency of sensor sampling rate. This introduces inconsistency across data sessions used for a labeled human activity. Furthermore, data collection in the wild produces imbalanced and heterogeneous datasets across mobile devices and across human activities. These challenges can cause a distortion in computing gradients in the FL system, given each device’s local data. This is expected to significantly reduce the model performance in an FL setting. This section will illustrate these challenges and our solutions to mitigate their effect.  

\subsection{Data collection and data description}

Data collection overview: To get smartphone sensor data “in the wild,” we opted to collect data utilizing university students as subjects for the following reasons: (1) University students should have relatively good access to the smartphones and related technologies; (2) University students should be more credible and easier to be motivated than other sources (e.g. recruiting test subjects on crowd-sourcing websites); and (3) It will be easier for our team to recruit and distribute rewards to students. We launched two data collection runs for two months each, with a privately distributed data collection app from a third-party start-up. 
% first run at New Jersey Institute of Technology (NJIT) and the second run at Kent State University (KENT). 
% We collaborated with Unknot.id, a third-party start-up, to rapidly develop and deploy the data collection app. We performed two data collection runs, one at NJIT (starting mid-April) and one in KENT (starting mid-May). Each run lasts about three months. 

% App details: Our team worked closely with Unknot.id during all stages of the app development, including requirement materializing, testing, debugging, and deploying. The main considerations when designing the app are: (1) The app should have full registration function, so that each user can have an account; (2) The app should have good coverage over types of sensors and labels, but still be quick and easy to operate; and (3) The app should have minimum impact on users’ daily life and the smartphone’s battery life. Due to licensing limitations, only the Android version of the app was eventually developed and was distributed privately instead of going through the app market. This limits the scope of the data collection to Android users.

% \begin{figure}[t!]
%   \centering
%   \begin{minipage}[b]{0.23\textwidth}
%   \includegraphics[width=\linewidth]{image/unknot1.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.23\textwidth}
%   \includegraphics[width=\linewidth]{image/unknot2.png}
%   \end{minipage}
%   \caption{Screenshots of Data Collection\label{unknot}}
% \end{figure}

% The app has two main components: (1) The frontend (i.e., the app itself on the phone, illustrated in Figure 1) for user interaction; and (2) The backend in the cloud that supports the data collection. The main functions of the app are: (1) Acquire sensor data from the smartphone; (2) Allow users to label their current/upcoming activities; (3) Detect user activities and reminds users to provide labels of their activities; and (4) Upload the collected data and labels to the backend. In addition, users could register their own accounts on the app, turn-off the types of data that they do not want to share, and track their upload history. 



Trade-offs between the sampling rate of sensor data and the impact on the smartphones’ battery life had to be made, which means the sensor data was sometimes not collected at the maximum available sampling rate. The differences between individual makes and models of Android smartphones also contributed to the variability and availability of the collected sensor data. In Table 2, we show the total number of minutes of data collected from the four types of sensors that collects continuous (relatively continuous compared with other sensors that collect data points at a much lower rate or at certain events) data sessions. We can see that only the Accelerometer collected a meaningful amount of data at the sampling rate higher than 5Hz. This also means that we may need to find means to temporally align data segments from different sensors with different sampling rates. Table 3 shows the number of data points collected from the rest of the sensors. Note that the Pressure sensor and the Light sensor collect data points at regular (but low) rates, while other sensors at certain events.

For the labels of activities, we summarized the labels into three categories: (1) Physical activity; (2) Phone position; and (3) User location. Each category has several pre-defined sub-types for users to choose from. The details can be seen in Table 4. From Table 4 we can see that: (1) Only several labels (“Recreational sports”, “Plane”, and “Shuttle”) were not collected by any participant, which could be partially due to the COVID-19 pandemic; (2) Also, the distribution of certain types of labels suggests the heavy influence that the COVID-19 pandemic had over people’s routine activities. This suggests that a comparison study between the data collected during the pandemic and the data collected during the “normal” time would be of great research value.

Instead of letting users freely report their activities, we provide a simple interface in the app for users to quickly select the appropriate labels, as shown in Figure 1. The combinations of labels will cover a vast majority of daily activities that are of research interests. Users can choose the labeling to last either for a defined time length (e.g., 5 minutes, 10 minutes, or 20 minutes) or for an unlimited time. In the second case, the users need to remember to turn off the label when the activity is done. 

As an attempt to further improve the temporal coverage of labels, we implemented a mechanism that detects user activities through existing Android means and notifies users to agree or disagree with the automatic labels, as well as to provide more detailed labels. This mechanism is employed only when the users are not actively providing labels. We implemented this mechanism utilizing the “Activity Recognition API” provided by Android. 
The list of activities that will be detected and labeled is provided in Table 5.

\begin{table}[]
\caption{Type of notifications and time covered}
\begin{tabular}{|l|l|}
\hline
Notification type & Total number of minutes covered by   notifications \\ \hline
Walking           & 5398.95                                            \\ \hline
Cycling           & 631.51                                             \\ \hline
Vehicle           & 11298.05                                           \\ \hline
\end{tabular}
\end{table}

The data and labels for each user are uploaded to the backend server that runs on a secure AWS instance fully managed by Unknot.id and NJIT. Upon registration, each account will get a unique random identifier for the user. The raw data and labels are associated only with this identifier to ensure user anonymity. The total size of the accumulated raw data is 700 GB. Table 6 shows the total amount of labels collected from the two data collection runs. Figure 2 shows an example of one-day overview of the sensor data collected from one user.

\begin{table}[]
\caption{Data overview}
\begin{tabular}{|l|l|}
\hline
Notification type & Total number of minutes covered by   notifications \\ \hline
Walking           & 5398.95                                            \\ \hline
Cycling           & 631.51                                             \\ \hline
Vehicle           & 11298.05                                           \\ \hline
\end{tabular}
\end{table}

\begin{figure}[t!]
  \centering
  \includegraphics[width=1\linewidth]{image/sensor_one_day.jpg}
  \caption{Example of sensor coverage of one user in one day}
%   \label{geolife_hm}
\end{figure}

\subsection{Data processing and statistical analysis}

The goal of data processing is to have the data ready to be consumed by the deep learning models. To be more specific, the processing steps need to achieve three objectives: (1) Remove or fix the errors and imperfections in the raw data, including repeated data points, gaps between data points, fluctuating sampling rates, and inaccurate labels. (2) Align the sensor data with the labels across time, such that each unit of data points is associated with its correct label; and (3) Convert the format of the raw data into short sessions of data points with multiple channels (i.e., accelerometer data has 3 channels, x, y, z, in the data representation) that will serve as basic input data units of the deep learning models. 
When working on the data, we found that objectives (2) and (3) were fairly easy to implement, but the unexpected quality issues in the data (due to the challenges mentioned at the beginning of Section 2) made achieving the objective (1) difficult. To recap, the major challenges are: (1) A big portion of motion sensor data (e.g., accelerometer and gyroscope) have unstable sampling rate and/or lower-than-expected sampling rate. This problem mainly comes from the way that the Android system provides sensor data and from the trade-offs that Unknot.id had to make when developing the app, and is difficult to be avoided; (2) Labels are not always reliable. Initial visual inspection of the labels revealed that some participants often forgot to turn-off the “unlimited time” labels, resulting in implausible labels (e.g. “sitting” for 10 hours straight). We also discovered completely “flat” sensor data segments associated with labels that should involve movements (e.g., “Walking” with the phone “In the pocket”). (3) The notification answers were also not reliable as conflicting answers (e.g., answering “Yes” to the notification, but providing different labels from the automatic ones in the notification) and implausible activity sequences (e.g., short sequences of “Driving” and “Cycling” repeatedly appear one after another); (4) Labels were highly imbalanced. This is mostly caused by the lockdown during the spread of the COVID-19 virus. Some “meaningful” labels (e.g., “Workout” and “Cycling”) were extremely rare, while some less interesting labels (e.g., “Lying”) were abundant.

Coping with the data challenges: We have tried many settings to deal with the data challenges. We first describe the solutions that we tried, which did not improve the model significantly. Then, we describe our current solution that works well. To validate that our model is not bad, we trained it on the UCI-HAR dataset [UCI] and achieved above 90\% classification accuracy without any optimization effort. Unlike our data, which is collected in the wild, the UCI-HAR dataset is collected in a controlled environment.
For the sampling rate issue, we tried first to down-sample all data points to 5Hz. However, this results in the loss of details and slows model response time (e.g., a 100-points data segment is 20 seconds long, which means the model cannot identify activities that last less than 20 seconds). Then, we tried to perform re-sampling on raw data (up-sampling of data with low sampling rates, and down-sampling of data with high sampling rate) with linear interpolation to convert them to the same intermediate sampling rate (e.g., 20Hz). This dataset suffers from the noise introduced by up-sampling (and also the loss of details from down-sampling). Therefore, we decided to stop re-sampling and switch to filtering to make sure the original data are of good quality. 
Then we were faced with the problem of “flat” data. The problem is that the flat data appears in data segments of all classes, which confuses the model. These flat data segments likely originated from either (1) Sampling issue by the Android system; or (2) Labeling errors due to the non-controlled nature of the data collection process. At first, we filtered the flat data at the session-level. However, after we examined the data segments, we found that even if a session is generally not “flat,” the individual data segments sampled from it can still be flat. Thus, we implemented segment-level flat data filtering.
We also tried to combine two sensors together (e.g., accelerometer and gyroscope, which is a popular combination in many HAR studies). The major step of doing so is to temporally align the data from the two sensors. First, we find one data session from each sensor with common sections and labels, e.g., in total, there are two parallel sessions for accelerometer and gyroscope. Then on each data session, we apply a sliding window to sample segments from both sessions at the same time. If two data sessions have the same sampling rate, then the two sliding windows will have the same overlapping rate. If the two data sessions have different sampling rates, then the two sliding windows are led by the one with lower sampling rate, which means that the sliding window on the lower sampling rate session will move forward with a higher overlapping rate (to generate more data segments), and the sliding window on the higher sampling rate session will follow the other window, in order to keep the sampled data segments temporally aligned (thus the segments on the higher sampling rate session will have relatively lower overlapping rate). Segments from two sensors were aligned as close as possible at their beginnings. However, introducing a second sensor in our case did not improve performance significantly. In some cases, it even caused more overfitting from the model. Thus, we opted to use only the accelerometer data at this stage of the project and leave sensor fusion for future work. 

Using only accelerometer data, our current data processing techniques consists of the following steps:
(1) Any duplicated data points (e.g., data points that have the same timestamp) are merged by taking the average of their sensor values.

(2) Using 300 milliseconds as the threshold, continuous data sessions are identified and separated by breaking up the data sequences at any gap that is larger than the threshold. This threshold is relatively strict, and it is defined based on the lowest effective sampling rate (5Hz) with some flexibility so that data sessions are not broken into too many pieces.

(3) Data sessions that have unstable or unsuitable sampling rates are filtered out. We only keep the data sessions that have a stable sampling rate of 5Hz or 20Hz or 50Hz. To achieve this, key statistics that are related to the sampling rate of each session, including the mean, the variance, and the 50\% quantile of the duration of gaps between consecutive data points, are computed. Then, the sessions that meet all of the following criteria are kept as potential valid data sessions: (a) The mean sampling rate (computed from mean gap duration) falls within ±25\% of the target sampling rates; (b) The 50\% quantile sampling rate (computed from 50\% quantile gap duration) falls within ±25\% of the target sampling rates; (c) The total duration exceeds 30 seconds. Here the assumption is that if the mean sampling rate and the 50\% quantile sampling rate agrees, it indicates that the data session has a relatively stable sampling rate. No resampling was done and all sessions are kept at their original sampling rate. 

(4) The label session(s) that are associated with each data session (if any) are identified from the raw labels data. Note that the label sessions are also filtered with the following two criteria to ensure good quality: (a) The first 10 seconds and the last 10 seconds of each label session are trimmed, due to the fact that users were likely operating the phone during these time periods; (b) Any label session longer than 30 minutes is trimmed down to 30 minutes, in order to mitigate the potential inaccurate labels due to users’ negligence (forgot to turn off labeling). We only use a subset of all the labels we collected (details are shown in Table 6). The notification labels were not used for now. 

(5) We sample data segments at the size of 100 data points with sliding windows. Different overlapping percentages were used for different classes and different sampling rates. The majority classes have 25\% overlapping to reduce the number of data segments, while the minority classes have up to 90\% overlapping to increase the available data segments. The same principle applies to sessions with different sampling rates. All data segments with different sampling rates are mixed together, without distinguishing between them. Our model has the capacity to learn from data with different sampling rates, thus reducing the computational cost of performing data processing on mobile devices. The training and testing data split is also done at this stage, with the guarantee that there is no overlapping between training data and testing data. We sample 15\% of data for testing, while the rest are used for training. To ease the sampling during FL training, training data are pre-split into chunks (size = 32) with approximately less than 10\% over-sampling. Testing data is saved as is. The statistics of the dataset are also shown in Table 7. 

\begin{table*}[]
  \caption{Statistics of the dataset for model training.}
\begin{tabular}{|l|l|l|l|l|}
\hline
Class            & Class index & Description                 & N training (100-points segments) & N testing (100-points segments) \\ \hline
Walking          & 0           & Walking                     & 49376                            & 8599                            \\ \hline
Sitting          & 1           & Sitting, exclude in vehicle & 52448                            & 8744                            \\ \hline
In-Vehicle, Car  & 2           & Driving or sitting          & 49536                            & 8586                            \\ \hline
Cycling          & 3           &                             & 14336                            & 2537                            \\ \hline
Workout, Running & 4           &                             & 1984                             & 319                             \\ \hline
\multicolumn{5}{|l|}{*All classes exclude phone position   = "Table"}                                                             \\ \hline
\end{tabular}
\end{table*}

(6) The sensor values in the training dataset and the testing dataset are normalized with z-score using the mean and standard deviation computed from the training dataset. This step is a common practice that helps to stabilize the gradients during training.

(7) Finally, we compute the mean-variance on each data segment with a rolling window (window size = 20), then filter out any data segment that has a variance value less than the threshold of 0.001. This step filters out the “flat” data segments. With this step, the data processing is completed.

All the reported model performance in Section 5 will be based on this dataset generated with the method above. In Figures 3, 4, and 5, some random samples of data segments of each class are shown. It is clear that different classes have different patterns, and there are no similar “flat” data segments in different classes to confuse the model.

\begin{figure}[t!]
  \centering
  \begin{minipage}[b]{0.23\textwidth}
  \includegraphics[width=\linewidth]{image/walking.png}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.23\textwidth}
  \includegraphics[width=\linewidth]{image/sitting.png}
  \end{minipage}
  \caption{Data segment samples. Left: Class 0 (“Walking”), Right: Class 1 (“Sitting”).}
\end{figure}

\begin{figure}[t!]
  \centering
  \begin{minipage}[b]{0.23\textwidth}
  \includegraphics[width=\linewidth]{image/driving.png}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.23\textwidth}
  \includegraphics[width=\linewidth]{image/cycling.png}
  \end{minipage}
  \caption{Data segment samples. Left: Class 0 (“Walking”), Right: Class 1 (“Sitting”).}
\end{figure}

\begin{figure}[t!]
  \centering
  \includegraphics[width=1\linewidth]{image/running.png}
  \caption{Data segment samples for Class 4 (“Running”)}
%   \label{geolife_hm}
\end{figure}
}

==> model_backup.tex <==
\begin{table*}[t]
\small
\centering
\caption{Types of Sensor Data Collected}
\begin{tabular}{|l|l|l|l|l|}
\hline
Sensor                             & Type                                    & Sampling rate                      & Availability                     & Description                                                                               \\ \hline
Accelerometer                      & Motion                           & 5Hz $\sim$50Hz                     & 114/116                          & Measures the linear acceleration   (including gravity)                                    \\
Gyroscope                          & Motion                           & 5Hz                                & 114/116                          & Measures the angular speed                                                                \\
Rotation                           & Motion                           & 5Hz                                & 114/116                          & Provides the rotation vector   component                                                  \\
GPS                                & Position                         & Variable                           & 110/116                          & Typical GPS data                                                                          \\
Magnetometer                       & Position                         & 5Hz                                & 113/116                          & Measures the geomagnetic field   strength                                                 \\
Pressure                           & Environment                      & 5Hz                                & 83/116                           & Measures ambient air pressure                                                             \\
Light                              & Environment                      & Variable                           & 110/116                          & Measures ambient light level   (illumination)                                             \\
Battery log                        & Phone state                      & Variable                           & 116/116                          & Measures the smartphone’s battery   level                                                 \\
Proximity                          & Phone state                      & Variable                           & 109/116                          & Measures the distance between the   screen and an object                                  \\
Power state                        & Phone state                      & Variable                           & 115/116                          & Different values indicating   different state/event of the smartphone                     \\
Call log                           & User data                               &                                    & 98/116                           & Logs the calls that the user had                                                          \\
SMS log                            & User data                               &                                    & 98/116                           & Logs the short messages (SMS) that   the user had                                         \\
\hline
\multicolumn{5}{|l|}{\begin{tabular}[c]{@{}l@{}}*The sampling rate is estimated   from observation, actual values vary\\ **The availability means that out   of the 116 participants, how many of them provided this data type 
\end{tabular}}
\\ \hline
\end{tabular}
\label{SensorData}
\end{table*}

\begin{table*}[]
\small
\centering
\caption{Total time of sensor sessions (continuous sensors)}
\begin{tabular}{|llllllll|}
\hline
Sensor        & Total\_time & 60hz\_up  & 50hz      & 40hz   & 20hz     & 5hz        & The\_rest \\ \hline
Accelerometer & 2278050.17  & 120056.98 & 241932.44 & 642.59 & 69136.15 & 1012894.06 & 833387.95 \\
Gyroscope     & 2273397.28  & 110149.8  & 15448.17  & 7.39   & 31354.51 & 1795766.05 & 320671.36 \\
Rotation      & 2290372.31  & 23073.62  & 71003.64  & 441.01 & 33341.33 & 2061158.39 & 101354.32 \\
Magnetometer  & 2287446.51  & 870.32    & 4058.21   & 0      & 23.01    & 2193983.48 & 88511.49  \\ \hline
\multicolumn{8}{|l|}{*In a number of minutes}                                                    \\
\multicolumn{8}{|l|}{**Only count data sessions at least   30 seconds long}                      \\ \hline
\end{tabular}
\label{SensorSessions}
\end{table*}

\section{HAR-Wild: Data, Models, and Training with FLSys}
\label{sec:model}
{\fontfamily{ptm}\selectfont

In order to demonstrate the efficiency and effectiveness of our FedSys, we carried out an end-to-end study on human activity recognition, including data collection in the wild, DL models, and FL training algorithms.



\subsection{Data Collection in the Wild}

Through our Data Collector, we collect smartphone sensor data (Table \ref{SensorData}) ``in the wild'' from university students as subjects for the following reasons: \textbf{(1)} University students  have relatively good access to the smartphones and related technologies; \textbf{(2)} University students should be more credible and easier to be motivated than other sources (e.g., recruiting test subjects on crowd-sourcing websites); and \textbf{(3)} It will be easier for our team to recruit and distribute rewards to students.
We launched two data collection runs at two universities for three months each. During the course of three months, we let the participants to collect data and labels by themselves (in the wild), and only intervene through reminding emails if we saw a decline in the amount of daily activities. A total of 116 participants were recorded after the two data collection runs. 

\begin{wrapfigure}{l}{0.18\textwidth}
  \begin{center} \vspace{-20pt}
    \includegraphics[width=0.2\textwidth]{image/Screenshot_anoymous.png} \vspace{-30pt}
  \end{center}
  \caption{Data Collector labeling interface.} \vspace{-10pt}
  \label{data_collector_labeling_interface}
\end{wrapfigure}

The types of data that the app can collect are listed in Table 1. The availability field marks how many of our student volunteers can collect each data type. In Table 2, we show the total number of minutes of data collected from the four types of sensors that collects continuous (relatively continuous compared with other sensors that collect data points at a much lower rate or at certain events) data sessions. We can see that only the Accelerometer collected a meaningful amount of data at the sampling rate higher than 5Hz. This also means that we may need to find means to temporally align data segments from different sensors with different sampling rates. Table 3 shows the number of data points collected from the rest of the sensors. Note that the Pressure sensor and the Light sensor collect data points at regular (but low) rates, while other sensors at certain events.

\begin{comment}
\begin{figure}[t!]
  \centering
  \includegraphics[width=0.4\linewidth]{image/Screenshot_anoymous.png}
  \caption{Data Collector labeling interface.}
  \label{data_collector_labeling_interface}
\end{figure}
\end{comment}



\begin{table}[t]
\small
\centering
\caption{Total number of data points (non-continuous sensors)}
\begin{tabular}{|l|l|}
\hline
Sensor     & Total number of data points \\ \hline
gps        & 1251970                     \\ \hline
pressure   & 971782334                   \\ \hline
light      & 380064951                   \\ \hline
batteryLog & 7721722                     \\ \hline
proximity  & 3280332                     \\ \hline
powerState & 794895                      \\ \hline
callLog    & 11362                       \\ \hline
textsLog   & 204728                      \\ \hline
\end{tabular}
\end{table}

\begin{table}[t]
\small
\caption{Labels and the total number of minutes collected for each label}
\begin{tabular}{|l|l|l|}
\hline
Type           & Label                        & Total minutes \\ \hline
Activity       & sitting                      & 862544.50     \\ \hline
               & walking                      & 158087.40     \\ \hline
               & driving                      & 38013.98      \\ \hline
               & lying                        & 488596.70     \\ \hline
               & cycling                      & 2589.50       \\ \hline
               & workout\_gym                 & 3649.47       \\ \hline
               & workout\_running             & 2212.69       \\ \hline
               & workout\_others              & 16500.13      \\ \hline
               & workout\_recreational sports & 0.00          \\ \hline
Phone position & palm                         & 511092.20     \\ \hline
               & bag                          & 6446.19       \\ \hline
               & pocket                       & 99557.67      \\ \hline
               & table                        & 864904.00     \\ \hline
               & mounted                      & 49440.29      \\ \hline
               & strap                        & 2485.22       \\ \hline
User location  & vehicle\_car                 & 72121.55      \\ \hline
               & vehicle\_train/subway        & 355.24        \\ \hline
               & vehicle\_plane               & 0.00          \\ \hline
               & vehicle\_bus/shuttle         & 0.00          \\ \hline
               & vehicle\_motorcycle          & 88.84         \\ \hline
               & home                         & 1171968.00    \\ \hline
               & outside                      & 41886.80      \\ \hline
               & travel                       & 14094.12      \\ \hline
               & elevator                     & 924.09        \\ \hline
               & office                       & 17562.08      \\ \hline
\end{tabular}
\label{DataActivities}
\end{table}

\begin{table}[t]
\small
\caption{Statistics of the dataset for model training.}
\label{tab:dataset}
\centering
\begin{tabular}{|l|l|l|}
\hline
Class   & N training & N testing \\ \hline
Walking      & ?????     & ?????       \\ \hline
Sitting, Not in vehicle  & ?????     & ?????   \\ \hline
In-Vehicle, Car (Driving, sitting)   & ?????  & ?????   \\ \hline
Cycling    & ?????    & ?????    \\ \hline
Workout, Running     & ?????   & ?????   \\ \hline
\multicolumn{3}{|l|}{*All classes exclude phone position   = ``Table''}                                                             \\ \hline
\end{tabular}
\end{table}

Regarding labels of activities, we provide a simple interface in our Data Collector for users to quickly select the appropriate labels, as shown in Figure \ref{data_collector_labeling_interface}. We summarized the labels into three categories: (1) Physical activity; (2) Phone position; and (3) User location. Each category has several pre-defined sub-types for users to choose from. The details can be seen in Table \ref{DataActivities}. Reported activities cover a vast majority of daily activities that are of research interests. Users can choose the labeling to last either for a defined time length (e.g., 5 minutes, 10 minutes, or 20 minutes) or for an unlimited time (i.e., in this case, users need to remember to turn off the label when the activity is done). We can see that the distribution of user activities is consistent with the ``stay home order" during the COVID-19 pandemic.

\subsection{Data Processing}

The goal of data processing is to have the data ready to be consumed by the deep learning models. Although our Data Collector is designed to be battery efficient, data collection in the wild, especially for human activity recognition (HAR), is noisy and more complicated than in well-controlled environments. This introduces inconsistency across data sessions used for a labeled human activity.


To cope with this challenge, the data processing steps need to achieve three objectives: \textbf{(1)} Remove or fix the errors and imperfections in the raw data, including repeated data points, gaps between data points, fluctuating sampling rates, and inaccurate labels; \textbf{(2)} Align the sensor data with the labels across time, such that each unit of data points is associated with its correct label; and \textbf{(3)} Convert the format of the raw data into short sessions of data points with multiple channels (i.e., accelerometer data has 3 channels, x, y, z, in the data representation) that will serve as basic input data units of the deep learning models. 

For the demonstration purpose, let us present our data processing techniques by using accelerometer data, as follows:  

(Step 1) Any duplicated data points (e.g., data points that have the same timestamp) are merged by taking the average of their sensor values.

(Step 2) Using 300 milliseconds as the threshold, continuous data sessions are identified and separated by breaking up the data sequences at any gap that is larger than the threshold. This threshold is relatively strict, and it is defined based on the lowest effective sampling rate (5Hz) with some flexibility so that data sessions are not broken into too many pieces.

(Step 3) Data sessions that have unstable or unsuitable sampling rates are filtered out. We only keep the data sessions that have a stable sampling rate of 5Hz or 20Hz or 50Hz. To achieve this, key statistics that are related to the sampling rate of each session, including the mean, the variance, and the 50\% quantile of the duration of gaps between consecutive data points, are computed. Then, the sessions that meet all of the following criteria are kept as potential valid data sessions: (a) The mean sampling rate (computed from mean gap duration) falls within ±25\% of the target sampling rates; (b) The 50\% quantile sampling rate (computed from 50\% quantile gap duration) falls within ±25\% of the target sampling rates; (c) The total duration exceeds 30 seconds. Here the assumption is that if the mean sampling rate and the 50\% quantile sampling rate agrees, it indicates that the data session has a relatively stable sampling rate. No resampling was done and all sessions are kept at their original sampling rate. 

(Step 4) The label session(s) that are associated with each data session (if any) are identified from the raw labels data. Note that the label sessions are also filtered with the following two criteria to ensure good quality: (a) The first 10 seconds and the last 10 seconds of each label session are trimmed, due to the fact that users were likely operating the phone during these time periods; (b) Any label session longer than 30 minutes is trimmed down to 30 minutes, in order to mitigate the potential inaccurate labels due to users’ negligence (forgot to turn off labeling). 

(Step 5) We sample data segments at the size of 100 data points with sliding windows. Different overlapping percentages were used for different classes. The majority classes have 25\% overlapping to reduce the number of data segments, while the minority classes have up to 90\% overlapping to increase the available data segments. The same principle applies to sessions with different sampling rates. All data segments with different sampling rates are mixed together, without distinguishing between them. We sample 15\% of data for testing, with the guarantee that no overlap between training and testing data exists. The rest 85\% of data points are used for training. The statistics of the dataset are also shown in Table \ref{tab:dataset}.

(Step 6) The sensor values in the training dataset and the testing dataset are normalized with z-score using the mean and standard deviation computed from the training dataset. This step is a common practice that helps to stabilize the gradients during training.

(Step 7) Finally, we compute the mean-variance on each data segment with a rolling window (window size = 20), then filter out any data segment that has a variance value less than the threshold of 0.001. This step filters out the “flat” data segments that are labeling errors. With this step, the data processing is completed.

The processed dataset will be used to evaluate model and system performance in this study.

\subsection{HAR-Wild Model and Training}

Our HAR-Wild model is designed to be efficiently trained on mobile devices for federated learning, given its small size, easy training, and high performance, compared with other computationally expensive models, such as LSTMs.
%We propose one model, FL-CNN, which can use either centralized training or federated training. 
Our model has three convolutional layers and a dense layer (Figure \ref{arch}).
To leverage the recipe of ResNet model into a tiny model for FL on mobile devices, HAR-Wild uses accelerometer data as input of (1) a sequence of 1D-CNN - Batch Norm - 1D-CNN - Batch Norm - Flatten layers, and (2) a sequence of 1D-CNN - Batch Norm - Flatten layers. The two flatten layers are concatenated before feeding them into a sequence of Drop Out - Dense - Output layers. By doing this, HAR-Wild is able to memorize and transfer the low latent features learned from the very first 1D-CNN, which is directly derived from the input data, to the output layer for better classification. 

\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{image/model.png}
  \caption{HAR-Wild model.}
  \label{arch}
%   \vspace{-0.15in}
\end{figure}

In centralized training, we use typical optimizers, such as Adam \cite{}, to train HAR-Wild. In federated training, we propose a data augmentation algorithm, called \textbf{Uniform Augmentation}, to address the non-IID issue. Our goal is to mitigate the distortion in computing gradients at client-side, without introducing bias toward a particular class in the training process. To achieve this goal, at the client-side, our idea is to augment the local data by providing a small number of data points of missing classes for each client.
We first collect a small number of random samples for each class, which will be used for data argumentation (Line 3, Algorithm \ref{alg_uniform_aug}). In each communication round, the algorithm simply combines the augmentation data with the local data to compute the local gradients at a particular client (Lines 9 and 10, Algorithm \ref{alg_uniform_aug}). The local gradients are then sent to the cloud for a typical average aggregation and a model update (Lines 11 and 12, Algorithm \ref{alg_uniform_aug}).


To avoid unnecessary privacy leakage in practice, augmentation data can be collected 1) given a small volunteer or controlled participants, or 2) by using publicly available data sets. In order to deliver the augmentation data to the clients, there are two approaches for two criteria: (1) privacy-preserving, and (2) communication efficiency. To provide better communication efficiency, we only need to send augmentation data regarding missing classes to the clients. In this approach, we need to know which classes are missing for each client. This introduces an additional privacy concern. In order to address this, in the second approach, we first deliver the entire augmentation data to every client, which is also practical given a small size of the data augmentation. Then, the unnecessary augmentation data is deleted after a local check at the client-side. This approach is better for privacy, but it transfers a little bit more data to mobiles.
In this study, we use the second approach to avoid additional privacy leakage. However, it can be replaced by the first approach, depending on the real-world application.

\begin{algorithm}
    \small
    \label{alg_uniform_aug}
	\caption{Uniform Augmentation} 
	\begin{algorithmic}[1]
	    \Procedure{Init}{}
    	    \State Clients pool $\mathcal{C}$
    	    \State Argumentation pool $\mathcal{A}$ = \Call{SampleArgumentationData}{$\mathcal{C}$}
    	    \State $Server\_model$ = \Call{InitServerModel}{ }
	    \EndProcedure
	    \Procedure{Training}{}
	        \For{number of rounds}
	            \State $Round\_clients$ = \Call{SampleClients}{$\mathcal{C}$} \Comment{each $client$ is ($id$, $data$)}
	            \State \Call{InitClientModels}{$Server\_model$}
	            \For{Each $client$ in $Round\_clients$}
	                \State $client.data$ = \Call{Concatenate}{$client.data$, $\mathcal{A}$}
	            \EndFor
	            \State $Client\_models$ = \Call{FedTraining}{$Round\_clients$}
	            \State $Server\_model$ =  \Call{FedAvg}{$Client\_models$}
	        \EndFor
	    \EndProcedure
	\end{algorithmic} 
\end{algorithm}

\begin{comment}
\subsubsection{Baseline Approaches}

We consider five baseline algorithms leveraging state-of-the-art works in FL for experimental evaluation, as follows: \textbf{(1)} \textbf{FedAvg} [McMahan et al., 2017] \cite{}, in which the average gradient, computed from an aggregation of all the gradients from clients in each round, is used to update the global model; \textbf{(2)} \textbf{FedProx} [Sahu et al., 2020], in which a regularization (Eq. \ref{regula}) is introduced to mitigate the gradient distortion from each client. The objective function at each local client is defined as follows:
\begin{equation} 
L(w,w^k)=F_k (w) + \mu/2 \lVert w-w^k\rVert_2
\label{regula}
\end{equation}
where $w$ is the value of the global model parameter. This restricts the divergence of parameters between clients that will arise due to heterogeneity in their data distributions, and (ii) For an appropriate choice of $\mu$, it will turn a non-convex loss function $F_k(w)$ into a convex $L(w,w^k)$ function, which is easier to optimize; \textbf{(3)} In each communication round, \textbf{Ensemble training} [Duan et al., 2021] (Algorithm \ref{}) selects the best local model among (i) all the local models derived from the clients and (ii) the aggregation of local models, based on their performance on a validation set, to be the global model in the cloud. The validation set can be a small random set of data points collected from all the clients; \textbf{(4)} \textbf{Ensembled Uniform Augmentation}, which is a combination of our Uniform Augmentation with the Ensemble training; and \textbf{(5)} \textbf{Ensembled Targeted Augmentation}, which is a combination of our Targeted Augmentation with the Ensemble training.

 \begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{image/alg3.png}
\end{figure}

\end{comment}

}

==> sec7_data_collection.tex <==
\vspace{-5pt}

\section{Appendix: HAR Data Collector} \vspace{-2.5pt}
\label{sec:data_collection}
% {\fontfamily{ptm}\selectfont

\subsection{Data Collection}

% \begin{wrapfigure}{l}{0.18\textwidth}
%   \begin{center} \vspace{-20pt}
%     \includegraphics[width=0.2\textwidth]{image/Screenshot_anoymous.png} \vspace{-30pt}
%   \end{center}
%   \caption{Data Collector labeling interface.} \vspace{-10pt}
%   \label{data_collector_labeling_interface}
% \end{wrapfigure}

Through our Data Collector app, %we collect smartphone sensor data (Table \ref{SensorData}) ``in the wild'' from university students. 
%as subjects for the following reasons: \textbf{(1)} University students have relatively good access to the smartphones and related technologies; \textbf{(2)} University students should be more credible and easier to be motivated than other sources (e.g., recruiting test subjects on crowd-sourcing websites); and \textbf{(3)} It will be easier for our team to recruit and distribute rewards to students. %\textcolor{red}{[We may remove the explanation to use university students if we need to cut size, or to remove less relevant info]}
we launched two sensor data collection runs at two universities for 4 months. We asked the participants to allow the app to collect data in the background and label some data  themselves. A total of 116 participants with valid data were recorded after the two data collection runs. The types of data that the app can collect are listed in Table \ref{SensorData}.


\begin{comment}
\begin{figure}[t!]
  \centering
  \includegraphics[width=0.4\linewidth]{image/Screenshot_anoymous.png}
  \caption{Data Collector labeling interface.}
  \label{data_collector_labeling_interface}
\end{figure}
\end{comment}


\begin{comment}
\begin{table}[t]
\small
\centering
\caption{Total number of data samples}
\begin{tabular}{|l|l|}
\hline
Sensor     & Total number of data samples \\ \hline
gps        & 1251970                     \\ \hline
pressure   & 971782334                   \\ \hline
light      & 380064951                   \\ \hline
batteryLog & 7721722                     \\ \hline
proximity  & 3280332                     \\ \hline
powerState & 794895                      \\ \hline
callLog    & 11362                       \\ \hline
textsLog   & 204728                      \\ \hline
\end{tabular}
\end{table}
\end{comment}

Regarding labels of activities, we provide a simple interface in our Data Collector app to quickly select the appropriate labels.
%(Figure \ref{data_collector_labeling_interface}). 
We summarize the labels into three categories: \textbf{(1)} Physical activity; \textbf{(2)} Phone position; and \textbf{(3)} User location. The reported activities cover a vast majority of daily activities that are of research interests. Each category has several pre-defined sub-types for users to choose from. The details of all labels can be seen in Table~\ref{DataActivities}. Users can choose the labeling to last either for a defined time length (e.g., 5 minutes, 10 minutes, or 20 minutes) or for an unlimited time (i.e., in this case, users need to remember to turn off the label when the activity is done). %We can see that the distribution of user activities is consistent with the ``stay home order'' during the COVID-19 pandemic.

\subsection{Data Processing}

To cope with inconsistent labels caused by the sampling rates in our Data Collector, we design the data processing with three objectives in mind: \textbf{(1)} Fix or mitigate the errors and imperfections in the raw sensor data, including gaps, repetitive samples and fluctuating sampling rates; \textbf{(2)} Identify and remove inconsistency in the labels; and \textbf{(3)} Convert the raw data into short segments of data points with shape $[3, 100]$, that are the basic input data units for DL models, where each data segment consists of 100 3-axis data points of Accelerometer data. The processing steps are as follows: 

\textbf{(1)} Any duplicated data points are merged by taking the average of their sensor values;

\textbf{(2)} Using 300 milliseconds as the threshold, continuous data sessions are identified and separated by breaking up the data sequences at any gap that is larger than the threshold;

\textbf{(3)} Data sessions that have unstable or unsuitable sampling rates are filtered out. We keep the data sessions that have a stable sampling rate of 5Hz, 10Hz, 20Hz, or 50Hz; 

\textbf{(4)} The label sessions that are associated with each data session (if any) are identified from the raw labels. Note that the label sessions are also filtered with the following two criteria to ensure good quality: (a) The first 10 seconds and the last 10 seconds of each label session are trimmed, due to the fact that users were likely operating the phone during these time periods; (b) Any label session longer than 30 minutes is trimmed down to 30 minutes, in order to mitigate the potential inaccurate labels due to users’ negligence (forgot to turn off labeling); %We only use a subset of all the labels we collected (details are shown in Table \ref{tab:dataset}).

\textbf{(5)} We sample data segments at the size of 100 data points with sliding windows. Different overlapping percentages were used for different classes and different sampling rates. The majority classes have 25\% overlapping to reduce the number of data segments, while the minority classes have up to 90\% overlapping to increase the available data segments. 
%The same principle is applied to sessions with different sampling rates. All data segments with different sampling rates are mixed together, without distinguishing between them. 
We sample 15\% of data for testing, while the rest are used for training (Table \ref{table_dataset});

\textbf{(6)} All the sensor values are normalized with z-score using the mean and standard deviation computed from the training dataset. This step is a common practice that helps to stabilize the gradients during training;

\textbf{(7)} Finally, we compute the mean-variance on each data segment with a rolling window (window size = 20), then filter out any data segment that has a variance value less than the threshold of 0.001. This step filters out the “flat” data segments that are labeling errors.
%(since all of our classes represents some type of movement).


\begin{comment}
\begin{itemize}
    \item Step 1: Any duplicated data points (e.g., data points that have the same timestamp) are merged by taking the average of their sensor values.
    \item Step 2: Using 300 milliseconds as the threshold, continuous data sessions are identified and separated by breaking up the data sequences at any gap that is larger than the threshold. This threshold is relatively strict, and it is defined based on the lowest effective sampling rate (5Hz) with some flexibility so that data sessions are not broken into too many pieces.
    \item Step 3: Data sessions that have unstable or unsuitable sampling rates are filtered out. We only keep the data sessions that have a stable sampling rate of 5Hz or 20Hz or 50Hz. To achieve this, key statistics that are related to the sampling rate of each session, including the mean, the variance, and the 50\% quantile of the sampling intervals, are computed. Then, the sessions that meet all of the following criteria are kept as potential valid data sessions: (a) The mean sampling rate (computed from mean sampling interval) falls within ±25\% of the target sampling rates; (b) The 50\% quantile sampling rate (computed from 50\% quantile sampling interval) falls within ±25\% of the target sampling rates; (c) The total duration exceeds 30 seconds. Here the assumption is that if the mean sampling rate and the 50\% quantile sampling rate agrees, it indicates that the data session has a relatively stable sampling rate. We keep each data session at their original sampling rate.
    \item Step 4: The label session(s) that are associated with each data session (if any) are identified from the raw labels data. Note that the label sessions are also filtered with the following two criteria to ensure good quality: (a) The first 10 seconds and the last 10 seconds of each label session are trimmed, due to the fact that users were likely operating the phone during these time periods; (b) Any label session longer than 30 minutes is trimmed down to the first 30 minutes, in order to mitigate the potential inaccurate labels due to users’ negligence (forgot to turn off labeling).
    \item Step 5: We sample data segments at the size of 100 data points with sliding windows. Different overlapping percentages were used for different classes. The majority classes have 25\% overlapping, while the minority classes have up to 90\% overlapping. All data segments with different sampling rates are mixed together, without distinguishing between them. We sample 15\% of data for testing, with the guarantee that training and testing data never overlaps. The rest 85\% of data points are used for training. The statistics of the dataset are also shown in Table \ref{tab:dataset}.
    \item Step 6: All the sensor values are normalized with z-score using the mean and standard deviation computed from the training dataset. This step is a common practice that helps to stabilize the gradients during training.
    \item Step 7: Finally, we compute the mean-variance on each data segment with a rolling window (window size = 20), then filter out any data segment that has a variance value less than the threshold of 0.001. This step filters out the “flat” data segments that are labeling errors (since all of our classes represents some type of movement).
\end{itemize}
\end{comment}

